Experimental Design for Active Transductive Inference in Large Language Models

One emergent ability of large language models (LLMs) is that query-specific examples can be included in the prompt at inference time. In this work, we use active learning for adaptive prompt design and call it Active In-context Prompt Design (AIPD). We design the LLM prompt by adaptively choosing few-shot examples from a training set to optimize performance on a test set. The training examples are initially unlabeled and we obtain the label of the most informative ones, which maximally reduces uncertainty in the LLM prediction. We propose two algorithms, GO and SAL, which differ in how the few-shot examples are chosen. We analyze these algorithms in linear models: first GO and then use its equivalence with SAL. We experiment with many different tasks in small, medium-sized, and large language models; and show that GO and SAL outperform other methods for choosing few-shot examples in the LLM prompt at inference time.

==> ablation.tex <==
\subsection{Extensive ablation experiments with \greedy}
In this section we conduct an ablation study for various versions of \greedy. 


\textbf{\greedyxx:} This is the version implemented in the paper in all experiments which we call as \greedy. For clarity in this section, we will call this as \greedyxx. Recall the \greedyxx\ implemented in \Cref{sec:experimental setup} is as follows:
%
The chosen point in round $t$ aligns the most with the target point $\bx_*$ such that $I_t \gets \argmax_{i \in \cU_t} \bx_*\T \bx_i$. For multiple target points $\bx_{*,k}$ \greedyxx\ chooses $I_t \gets \argmax_{i \in \cU_t}\max_{k} \bx_{*,k}\T \bx_i$. 


\textbf{\greedymx:} The \greedymx\ works as follows:
%
The chosen point in round $t$ aligns the most with the target point $\bx_*$ such that $I_t \gets \argmax_{i \in \cU_t} \bx_*\T \bx_i$. For multiple target points $\bx_{*,k}$ \greedymx\ chooses $I_t \gets \argmax_{i \in \cU_t}\min_{k} \bx_{*,k}\T \bx_i$. 



\textbf{\greedymu:} Before we state this method, we define the notation $\mathrm{avg}(\bx_i) = \frac{1}{K}\sum_{k=1}^K \bx_{*,k}\T \bx_i$. Then define the score for a point $\bx_i$ with respect to $\bx_*$ and the distance from the average $\mathrm{avg}(\bx_i)$ as $s(\bx_i, \bx_*) =| \bx_*\T \bx_i - \mathrm{avg}(\bx_i)|$.
%
Now, the \greedymu\ works as follows:
%
At round $t$ choose a point that aligns most with the target point $\bx_*$. So the point is chosen such that $I_t \gets \argmax_{i \in \cU_t} \bx_*\T \bx_i$. For multiple target points $\bx_{*,k}$ \greedymu\ chooses $I_t \gets \argmax_{i \in \cU_t} \argmin_{k} s(\bx_i, \bx_{*,k})$. 
%
Observe that the inner $\min$ chooses the point $\bx_i$ closest to the average of all the target points $\bx_{*,k}$ to balance exploration.

\textbf{\dopt:} This baseline is motivated by the D-optimal design \citep{pukelsheim2006optimal,fedorov2013theory}. At round $t$, \dopt\ computes a distribution over unlabeled points $\cU_t$, $\pi_t = \argmax_\pi \log\det(\sum_{i \in \cU_t} \pi(i) \bx_i \bx_i^\top)$. The next point is chosen as $I_t \sim \pi_t$. We choose this baseline to show that other optimal design approaches are not as efficient as \go. Following \citet{kiefer1960equivalence, lattimore2020bandit}, we note that \dopt\ can also be viewed as $\pi_t = \argmin_\pi \max_{j \in \U_t} \bx_j^\top (\sum_{i \in \U_t} \pi(i) \bx_i \bx_i^\top)^{-1} \bx_j$. This shows the key difference from \eqref{eq:greedy go}. While \go\ minimizes the uncertainty of the target point $\bx_*$ only, \dopt\ does it for all points in $\cU_t$.


\begin{figure}[!ht]
\centering
\begin{tabular}{cc}
\subfigure[Classification on ARC Expansion and Contraction Experiment]{\includegraphics[scale = 0.35]{img/ablation/arc_expansion_contraction.png}\label{fig:ablation-1}} &
%%%%%%%%%%
\subfigure[Classification on ARC Rotation Experiment]{\includegraphics[scale = 0.35]{img/ablation/arc_ablation_rotation.png}\label{fig:ablation-2}}  \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%
\subfigure[Classification on PCFG Add Subtract]{\includegraphics[scale = 0.35]{img/ablation/pcfg_ablation.png}\label{fig:ablation-3}} &
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfigure[Classification on Iris]{\includegraphics[scale = 0.35]{img/ablation/iris_ablation_mis_class.png}\label{fig:ablation-4}} 
\end{tabular}
%\vspace{-1.2em}
\caption{Experiment results with Falcon 40B on ARC, PCFG, classification tasks. For the classification tasks, we show the cumulative mis-classification error in the y-axis.} 
\label{fig:expt-ablation}
\end{figure}

The experiments with all these variants are shown in \Cref{fig:expt-ablation}. From this \Cref{fig:expt-ablation} we see that none of the variants of the \greedy\ are reducing the misclassification error or 0-1 error as fast as \go\ or \sal. This performance of the many variants of \greedy\ can be attributed to its lack of correctly balancing exploration-exploitation.


\subsection{ Instructor embedding vs numerical features}
Instructor embedding can be derived for any inputs that can be represented as strings. In this section, we examine whether Instructor embedding is helpful in active experiment design when numerical input features are considered. As shown in \Cref {fig:instruct-ablation}, using Instructor embedding for the numerical features always hurts the performance of G-optimal active experiment design.

\begin{figure*}[t]
\centering
\includegraphics[scale = 0.32]{img/figure7.pdf}
\caption{Comparison of the cumulative error for active experiment design conducted with original numerical features vs. with Instructor embedding. The selected datasets all use numerical input features rather than natural language. \go\ is used in all the experiments in this figure.} 
\label{fig:instruct-ablation}
\end{figure*}



% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%          & Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $12.40 \pm 1.13$ & $11.00 \pm 0.55$ & $\mathbf{8.80 \pm 0.85}$ & $15.00 \pm 1.22$ & $10.10 \pm 0.73$ & $14.80 \pm 1.11$\\
% banknote& $10.70 \pm 0.62$ & $10.60 \pm 0.90$ & $11.20 \pm 0.12$ & $10.20 \pm 1.08$ & $\mathbf{9.30 \pm 0.92}$ & $10.60 \pm 0.70$\\
% balance-scale& $12.10 \pm 1.56$ & $\mathbf{9.60 \pm 0.70}$ & $14.70 \pm 1.64$ & $13.50 \pm 1.70$ & $11.00 \pm 0.65$ & $\mathbf{10.00 \pm 0.47}$\\
% thyroid-new& $12.50 \pm 1.15$ & $12.90 \pm 0.48$ & $13.10 \pm 1.73$ & $13.90 \pm 1.71$ & $13.20 \pm 0.44$ & $\mathbf{11.50 \pm 0.89}$\\
% movie& $13.00 \pm 0.67$ & $\mathbf{12.70 \pm 0.82}$ & $15.90 \pm 0.58$ & $15.00 \pm 0.85$ & $13.30 \pm 0.77$ & $13.70 \pm 0.93$\\
% theme& $14.50 \pm 0.52$ & $12.70 \pm 1.01$ & $15.90 \pm 0.73$ & $14.70 \pm 1.03$ & $13.00 \pm 1.27$ & $\mathbf{10.50 \pm 0.72}$\\
% entity& $13.70 \pm 1.12$ & $\mathbf{11.30 \pm 0.87}$ & $16.00 \pm 1.21$ & $15.20 \pm 1.31$ & $12.10 \pm 0.91$ & $13.10 \pm 1.69$\\
% machine(e+04)& $4.66 \pm 1.43$ & $\mathbf{2.61 \pm 1.15}$ & $10.3 \pm 1.10$ & $6.06 \pm 1.51$ & $3.09 \pm 1.08$ & $6.59 \pm 1.76$\\
% fifa(e+03)& $\mathbf{2.71 \pm 1.42}$ & $2.71 \pm 1.93$ & $6.28 \pm 3.71$ & $10.3 \pm 4.38$ & $3.07 \pm 1.46$ & $104 \pm 98.1$\\
%     \end{tabular}
%     \caption{Falcon-7B}
%     \label{tab:Falcon-7B}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%          & Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $12.40 \pm 1.13$ & $14.80 \pm 1.11$ & $\mathbf{8.80 \pm 0.85}$ & $15.00 \pm 1.22$ & $10.10 \pm 0.73$ & $11.00 \pm 0.55$\\
% banknote& $10.70 \pm 0.62$ & $10.60 \pm 0.70$ & $11.20 \pm 0.12$ & $10.20 \pm 1.08$ & $\mathbf{9.30 \pm 0.92}$ & $10.60 \pm 0.90$\\
% balance-scale& $12.10 \pm 1.56$ & $10.00 \pm 0.47$ & $14.70 \pm 1.64$ & $13.50 \pm 1.70$ & $11.00 \pm 0.65$ & $\mathbf{9.60 \pm 0.70}$\\
% thyroid-new& $12.50 \pm 1.15$ & $\mathbf{11.50 \pm 0.89}$ & $13.10 \pm 1.73$ & $13.90 \pm 1.71$ & $13.20 \pm 0.44$ & $12.90 \pm 0.48$\\
% movie& $13.00 \pm 0.67$ & $13.70 \pm 0.93$ & $15.90 \pm 0.58$ & $15.00 \pm 0.85$ & $13.30 \pm 0.77$ & $\mathbf{12.70 \pm 0.82}$\\
% theme& $14.50 \pm 0.52$ & $\mathbf{10.50 \pm 0.72}$ & $15.90 \pm 0.73$ & $14.70 \pm 1.03$ & $13.00 \pm 1.27$ & $12.70 \pm 1.01$\\
% entity& $13.70 \pm 1.12$ & $13.10 \pm 1.69$ & $16.00 \pm 1.21$ & $15.20 \pm 1.31$ & $12.10 \pm 0.91$ & $\mathbf{11.30 \pm 0.87}$\\
% machine(e+04)& $4.66 \pm 1.43$ & $6.59 \pm 1.76$ & $10.3 \pm 1.10$ & $6.06 \pm 1.51$ & $3.09 \pm 1.08$ & $\mathbf{2.61 \pm 1.15}$\\
% fifa(e+03)& $\mathbf{2.71 \pm 1.42}$ & $104 \pm 98.1$ & $6.28 \pm 3.71$ & $10.3 \pm 4.38$ & $3.07 \pm 1.46$ & $\mathbf{2.71 \pm 1.93}$\\
% \end{tabular}
%     \caption{Falcon-7B}
%     \label{tab:Falcon-7B-1}
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%          &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $6.20 \pm 0.64$ & $6.50 \pm 0.52$ & $5.80 \pm 0.46$ & $7.00 \pm 0.61$ & $5.60 \pm 0.87$ & $\mathbf{5.10 \pm 0.43}$\\
% banknote& $6.00 \pm 0.57$ & $\mathbf{4.40 \pm 0.58}$ & $6.30 \pm 0.34$ & $4.70 \pm 0.46$ & $6.10 \pm 0.29$ & $6.40 \pm 0.24$\\
% balance-scale& $6.40 \pm 0.68$ & $6.70 \pm 0.41$ & $7.10 \pm 0.66$ & $5.90 \pm 0.48$ & $\mathbf{5.30 \pm 0.64}$ & $7.10 \pm 0.62$\\
% thyroid-new& $5.70 \pm 0.62$ & $6.70 \pm 0.37$ & $\mathbf{5.00 \pm 0.79}$ & $6.50 \pm 0.87$ & $6.00 \pm 0.84$ & $5.40 \pm 0.43$\\
% movie& $7.60 \pm 0.33$ & $8.30 \pm 0.37$ & $7.80 \pm 0.73$ & $8.10 \pm 0.29$ & $\mathbf{7.20 \pm 0.46}$ & $7.20 \pm 0.64$\\
% theme& $7.00 \pm 0.39$ & $\mathbf{5.00 \pm 0.65}$ & $7.50 \pm 0.50$ & $8.70 \pm 0.46$ & $7.90 \pm 0.37$ & $5.70 \pm 1.02$\\
% entity& $7.90 \pm 0.75$ & $\mathbf{7.20 \pm 1.06}$ & $7.40 \pm 0.78$ & $8.00 \pm 0.45$ & $\mathbf{7.20 \pm 0.54}$ & $8.00 \pm 0.52$\\
% machine (e+04)& $1.70 \pm .410$ & $3.51 \pm 1.37$ & $4.63 \pm .748$ & $3.79 \pm 1.41$ & $1.02 \pm .309$ & $\mathbf{.711 \pm .217}$\\
% fifa(e+03)& $5.91 \pm 2.88$ & $1.38 \pm .59$ & $3.47 \pm 2.64$ & $1.43 \pm .657$ & $1.32 \pm .871$ & $\mathbf{1.21 \pm .524}$\\
% \end{tabular}
%     \caption{Falcon-40B}
%     \label{tab:Falcon-40B}
% \end{table}


% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%          &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $5.60 \pm 0.40$ & $6.60 \pm 0.33$ & $5.10 \pm 0.53$ & $6.90 \pm 0.43$ & $\mathbf{5.00 \pm 0.72}$ & $5.90 \pm 0.19$\\
% banknote& $5.20 \pm 0.25$ & $\mathbf{4.90 \pm 0.64}$ & $5.60 \pm 0.10$ & $5.10 \pm 0.29$ & $5.00 \pm 0.27$ & $6.20 \pm 0.44$\\
% balance-scale& $6.00 \pm 0.16$ & $7.10 \pm 0.66$ & $6.60 \pm 0.40$ & $5.90 \pm 0.70$ & $6.30 \pm 0.46$ & $\mathbf{5.60 \pm 0.46}$\\
% thyroid-new& $6.00 \pm 0.16$ & $6.90 \pm 0.24$ & $\mathbf{5.90 \pm 0.62}$ & $6.20 \pm 0.46$ & $6.00 \pm 0.47$ & $6.30 \pm 0.51$\\
% movie& $7.20 \pm 0.49$ & $7.50 \pm 0.42$ & $7.70 \pm 0.30$ & $9.00 \pm 0.27$ & $7.70 \pm 0.34$ & $\mathbf{6.90 \pm 0.29}$\\
% theme& $6.90 \pm 0.58$ & $\mathbf{5.70 \pm 0.66}$ & $8.50 \pm 0.42$ & $7.30 \pm 0.70$ & $6.40 \pm 0.48$ & $7.40 \pm 0.43$\\
% entity& $8.40 \pm 0.48$ & $8.10 \pm 0.29$ & $7.80 \pm 0.25$ & $8.20 \pm 0.30$ & $\mathbf{7.50 \pm 0.57}$ & $8.20 \pm 0.34$\\
% machine(e+04)& $1.88 \pm .569$ & $3.51 \pm 1.11$ & $5.07 \pm .727$ & $2.91 \pm .896$ & $.923 \pm .285$ & $\mathbf{.709 \pm .256}$\\
% fifa(e+03)& $5.23 \pm 3.59$ & $1.63 \pm .574$ & $4.38 \pm 3.55$ & $1.37 \pm .534$ & $\mathbf{.506 \pm .136}$ & $9.79 \pm 1.65$\\
% \end{tabular}
%     \caption{Falcon-40B}
%     \label{tab:Falcon-40B-1}
% \end{table}



% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $5.80 \pm 1.59$ & $\mathbf{4.60 \pm 1.35}$ & $11.30 \pm 1.81$ & $12.10 \pm 1.57$ & $6.10 \pm 1.96$ & $11.00 \pm 2.24$\\
% banknote& $7.60 \pm 0.40$ & $\mathbf{7.50 \pm 0.89}$ & $13.80 \pm 1.10$ & $10.00 \pm 0.00$ & $8.20 \pm 0.62$ & $10.00 \pm 0.00$\\
% balance-scale& $11.60 \pm 1.63$ & $11.20 \pm 0.25$ & $13.40 \pm 1.23$ & $10.40 \pm 0.43$ & $\mathbf{10.10 \pm 1.24}$ & $16.50 \pm 1.17$\\
% thyroid-new& $\mathbf{10.40 \pm 0.81}$ & $10.70 \pm 1.43$ & $11.60 \pm 1.76$ & $13.70 \pm 1.41$ & $11.20 \pm 1.01$ & $16.80 \pm 1.48$\\
% movie& $8.10 \pm 1.48$ & $\mathbf{7.00 \pm 0.76}$ & $10.90 \pm 1.43$ & $12.90 \pm 1.82$ & $7.90 \pm 1.33$ & $13.60 \pm 2.92$\\
% theme& $15.60 \pm 0.76$ & $12.10 \pm 1.50$ & $15.20 \pm 1.45$ & $15.20 \pm 1.21$ & $\mathbf{11.00 \pm 1.77}$ & $12.70 \pm 2.39$\\
% entity& $8.10 \pm 1.46$ & $7.90 \pm 1.97$ & $13.90 \pm 0.91$ & $17.00 \pm 1.23$ & $\mathbf{6.70 \pm 1.27}$ & $12.50 \pm 2.84$\\
% machine(e+04)& $6.72 \pm 1.97$ & $\mathbf{5.12 \pm 1.47}$ & $8.51 \pm 1.62$ & $6.35 \pm 1.75$ & $\mathbf{5.35 \pm 1.69}$ & $6.17 \pm 1.70$\\
% fifa(e+03)& $2.22 \pm .715$ & $\mathbf{1.25 \pm .340}$ & $1.51 \pm .419$ & $5.36 \pm 2.89$ & $\mathbf{1.37 \pm .325}$ & $5.34 \pm 2.47$\\
%     \end{tabular}
%     \caption{LLama2-7B}
%     \label{tab:LLama2-7B}
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $8.50 \pm 2.77$ & $22.20 \pm 3.27$ & $14.90 \pm 4.37$ & $23.00 \pm 3.78$ & $7.70 \pm 3.00$ & $\mathbf{6.30 \pm 3.68}$\\
% banknote& $11.40 \pm 1.62$ & $21.00 \pm 0.35$ & $28.80 \pm 1.62$ & $22.50 \pm 0.96$ & $14.30 \pm 2.19$ & $\mathbf{9.50 \pm 1.17}$\\
% balance-scale& $20.30 \pm 0.60$ & $31.50 \pm 3.50$ & $26.10 \pm 2.18$ & $19.70 \pm 4.27$ & $\mathbf{19.30 \pm 2.87}$ & $22.80 \pm 1.33$\\
% thyroid-new& $\mathbf{7.60 \pm 1.42}$ & $28.20 \pm 1.19$ & $14.50 \pm 3.09$ & $24.30 \pm 2.18$ & $16.30 \pm 0.98$ & $16.20 \pm 2.62$\\
% movie& $6.25 \pm 1.18$ & $29.65 \pm 4.94$ & $12.30 \pm 1.64$ & $33.25 \pm 2.67$ & $\mathbf{4.30 \pm 0.86}$ & $5.20 \pm 1.36$\\
% theme& $25.00 \pm 2.82$ & $23.50 \pm 3.63$ & $28.20 \pm 0.87$ & $31.30 \pm 2.22$ & $21.10 \pm 2.36$ & $\mathbf{20.20 \pm 2.20}$\\
% entity& $9.40 \pm 1.65$ & $35.40 \pm 2.51$ & $19.60 \pm 1.35$ & $34.60 \pm 2.28$ & $9.80 \pm 3.21$ & $\mathbf{8.30 \pm 3.39}$\\
% machine(e+04)& $11.4 \pm 3.34$ & $10.5 \pm 2.44$ & $14.3 \pm 3.39$ & $11.0 \pm 1.93$ & $\mathbf{10.5 \pm 3.74}$ & $10.6 \pm 3.84$\\
% fifa(e-04)& $1.40 \pm .216$ & $3.72 \pm 1.12$ & $1.18 \pm .535$ & $4.15 \pm 1.11$ & $.999\pm .404$ & $\mathbf{.680 \pm .262}$\\
% \end{tabular}
%     \caption{Mistral-7B}
%     \label{tab:Mistral-7B-1}
% \end{table}




% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $\mathbf{4.50 \pm 0.99}$ & $5.50 \pm 0.82$ & $9.30 \pm 0.97$ & $9.70 \pm 1.95$ & $6.40 \pm 1.00$ & $9.80 \pm 1.72$\\
% banknote& $9.70 \pm 0.75$ & $\mathbf{7.20 \pm 1.11}$ & $16.80 \pm 1.31$ & $10.30 \pm 0.64$ & $8.60 \pm 0.62$ & $9.60 \pm 0.70$\\
% balance-scale& $10.30 \pm 0.98$ & $10.50 \pm 1.08$ & $12.90 \pm 1.13$ & $\mathbf{9.60 \pm 2.18}$ & $11.80 \pm 0.58$ & $15.20 \pm 1.30$\\
% thyroid-new& $\mathbf{10.60 \pm 1.12}$ & $13.90 \pm 0.91$ & $12.90 \pm 0.93$ & $13.20 \pm 2.04$ & $12.20 \pm 0.34$ & $17.20 \pm 0.66$\\
% movie& $9.00 \pm 0.79$ & $\mathbf{8.80 \pm 0.66}$ & $11.60 \pm 0.80$ & $17.70 \pm 1.37$ & $10.50 \pm 1.24$ & $16.70 \pm 1.27$\\
% theme& $26.75 \pm 2.96$ & $22.25 \pm 2.08$ & $26.90 \pm 2.72$ & $31.20 \pm 2.13$ & $\mathbf{18.30 \pm 2.59}$ & $28.95 \pm 2.10$\\
% entity& $9.00 \pm 0.57$ & $\mathbf{8.30 \pm 0.93}$ & $11.50 \pm 1.39$ & $16.10 \pm 1.65$ & $9.60 \pm 0.56$ & $18.60 \pm 0.58$\\
% machine (e+04)& $6.27 \pm 1.78$ & $5.10 \pm 1.73$ & $7.13 \pm 1.95$ & $5.75 \pm 1.68$ & $4.83 \pm 1.84$ & $\mathbf{4.63 \pm 1.31}$\\
% fifa (e+03)& $2.40 \pm .674$ & $1.69 \pm .741$ & $1.45 \pm .250$ & $2.59 \pm 1.17$ & $\mathbf{.747 \pm 1.42}$ & $3.17 \pm 1.51$\\
% \end{tabular}
%     \caption{LLama2-13B}
%     \label{tab:LLama2-13B}
% \end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $6.60 \pm 1.35$ & $\mathbf{5.30 \pm 1.06}$ & $11.10 \pm 1.10$ & $12.50 \pm 1.28$ & $6.80 \pm 0.98$ & $9.70 \pm 1.19$\\
% banknote& $\mathbf{9.40 \pm 0.78}$ & $9.70 \pm 1.07$ & $13.50 \pm 0.76$ & $13.50 \pm 0.96$ & $11.60 \pm 0.51$ & $13.60 \pm 0.62$\\
% balance-scale& $11.90 \pm 2.14$ & $12.40 \pm 0.43$ & $12.40 \pm 1.08$ & $12.00 \pm 1.49$ & $\mathbf{11.30 \pm 1.21}$ & $16.10 \pm 0.53$\\
% thyroid-new& $\mathbf{10.60 \pm 0.43}$ & $12.30 \pm 0.85$ & $12.10 \pm 1.44$ & $14.10 \pm 1.96$ & $\mathbf{10.90 \pm 0.91}$ & $15.00 \pm 0.57$\\
% movie& $8.10 \pm 0.94$ & $6.50 \pm 1.04$ & $10.30 \pm 1.11$ & $16.80 \pm 0.86$ & $\mathbf{6.10 \pm 0.62}$ & $16.30 \pm 0.92$\\
% theme& $15.90 \pm 0.83$ & $17.20 \pm 1.41$ & $15.70 \pm 2.14$ & $16.20 \pm 1.85$ & $15.80 \pm 0.60$ & $\mathbf{14.00 \pm 1.33}$\\
% entity& $\mathbf{7.00 \pm 1.51}$ & $8.50 \pm 0.79$ & $13.90 \pm 1.13$ & $15.50 \pm 0.69$ & $9.30 \pm 1.53$ & $17.20 \pm 0.73$\\
% machine (e+04)& $5.59 \pm 1.35$ & $\mathbf{4.80 \pm 1.46}$ & $7.95 \pm 1.69$ & $4.98 \pm 1.06$ & $5.66 \pm 1.54$ & $5.04 \pm .851$\\
% fifa (e+03)& $5.90 \pm 1.59$ & $2.59 \pm .742$ & $5.11 \pm 1.12$ & $6.76 \pm 1.69$ & $\mathbf{1.44 \pm .258}$ & $4.72 \pm .931$\\
% \end{tabular}
%     \caption{Vicuna-13B}
%     \label{tab:Vicuna-13B}
% \end{table}




% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $6.60 \pm 1.35$ & $9.70 \pm 1.19$ & $11.10 \pm 1.10$ & $12.50 \pm 1.28$ & $6.80 \pm 0.98$ & $\mathbf{5.30 \pm 1.06}$\\
% banknote& $\mathbf{9.40 \pm 0.78}$ & $13.60 \pm 0.62$ & $13.50 \pm 0.76$ & $13.50 \pm 0.96$ & $11.60 \pm 0.51$ & $\mathbf{9.70 \pm 1.07}$\\
% balance-scale& $11.90 \pm 2.14$ & $16.10 \pm 0.53$ & $12.40 \pm 1.08$ & $12.00 \pm 1.49$ & $\mathbf{11.30 \pm 1.21}$ & $12.40 \pm 0.43$\\
% thyroid-new& $\mathbf{10.60 \pm 0.43}$ & $15.00 \pm 0.57$ & $12.10 \pm 1.44$ & $14.10 \pm 1.96$ & $10.90 \pm 0.91$ & $12.30 \pm 0.85$\\
% movie& $8.10 \pm 0.94$ & $16.30 \pm 0.92$ & $10.30 \pm 1.11$ & $16.80 \pm 0.86$ & $\mathbf{6.10 \pm 0.62}$ & $\mathbf{6.50 \pm 1.04}$\\
% theme& $15.90 \pm 0.83$ & $\mathbf{14.00 \pm 1.33}$ & $15.70 \pm 2.14$ & $16.20 \pm 1.85$ & $15.80 \pm 0.60$ & $17.20 \pm 1.41$\\
% entity& $\mathbf{7.00 \pm 1.51}$ & $17.20 \pm 0.73$ & $13.90 \pm 1.13$ & $15.50 \pm 0.69$ & $9.30 \pm 1.53$ & $8.50 \pm 0.79$\\
% machine(e+04)& $5.59 \pm 1.35$ & $5.04 \pm .851$ & $7.95 \pm 1.69$ & $4.98 \pm 1.06$ & $5.66 \pm 1.54$ & $\mathbf{4.80 \pm 1.46}$\\
% fifa(e+03)& $5.90 \pm 1.59$ & $4.72 \pm .931$ & $5.11 \pm 1.12$ & $6.76 \pm 1.69$ & $\mathbf{1.44 \pm .258}$ & $2.59 \pm .742$\\
% \end{tabular}
%     \caption{Vicuna-13B}
%     \label{tab:Vicuna-13B-1}
% \end{table}




% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\\hline
% iris& $4.80 \pm 1.42$ & $\mathbf{4.50 \pm 1.62}$ & $8.60 \pm 1.04$ & $11.20 \pm 2.12$ & $5.60 \pm 1.95$ & $10.80 \pm 2.03$\\
% banknote& $10.90 \pm 1.69$ & $9.20 \pm 0.98$ & $17.00 \pm 0.76$ & $11.20 \pm 0.62$ & $\mathbf{8.90 \pm 0.75}$ & $11.50 \pm 0.55$\\
% balance-scale& $11.40 \pm 1.93$ & $11.50 \pm 2.04$ & $11.70 \pm 1.66$ & $\mathbf{8.90 \pm 1.12}$ & $11.50 \pm 1.86$ & $15.80 \pm 2.37$\\
% thyroid-new& $8.00 \pm 1.48$ & $8.30 \pm 0.96$ & $10.00 \pm 2.91$ & $10.00 \pm 0.00$ & $\mathbf{7.80 \pm 0.64}$ & $13.50 \pm 2.14$\\
% movie& $2.40 \pm 0.68$ & $2.40 \pm 0.43$ & $8.50 \pm 1.64$ & $13.30 \pm 1.71$ & $\mathbf{2.20 \pm 0.49}$ & $10.40 \pm 0.99$\\
% theme& $16.00 \pm 1.12$ & $14.20 \pm 2.10$ & $13.50 \pm 1.42$ & $17.90 \pm 1.73$ & $\mathbf{12.40 \pm 2.60}$ & $15.40 \pm 2.86$\\
% entity& $\mathbf{3.60 \pm 0.64}$ & $3.60 \pm 1.09$ & $8.50 \pm 2.09$ & $18.50 \pm 1.14$ & $3.60 \pm 1.77$ & $15.30 \pm 2.19$\\
% machine(e+04)& $6.76 \pm 1.25$ & $5.85 \pm 1.99$ & $6.77 \pm .941$ & $3.62 \pm .428$ & $4.58 \pm 1.68$ & $\mathbf{3.47 \pm .545}$\\
% fifa(e+04)& $2.31 \pm .397$ & $\mathbf{1.65 \pm .473}$ & $2.33 \pm .850$ & $5.47 \pm .499$ & $1.76 \pm .269$ & $5.43 \pm .478$\\
% \end{tabular}
%     \caption{Math-DPO-13B}
%     \label{tab:Math-DPO-13B}
% \end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
% &Uniform & Greedy-NN & LC & Max-Ent & GO (ours) & SAL (ours)\\
% iris& $\mathbf{15.90 \pm 0.90}$ & $18.05 \pm 1.55$ & $19.70 \pm 0.53$ & $32.35 \pm 2.95$ & $19.45 \pm 1.74$ & $32.80 \pm 2.73$\\
% banknote& $20.00 \pm 0.64$ & $21.20 \pm 0.70$ & $\mathbf{18.60 \pm 0.94}$ & $21.00 \pm 1.29$ & $20.20 \pm 1.31$ & $20.30 \pm 0.31$\\
% balance-scale& $24.65 \pm 1.58$ & $23.65 \pm 1.24$ & $28.40 \pm 1.26$ & $28.30 \pm 3.36$ & $\mathbf{22.60 \pm 2.01}$ & $24.40 \pm 2.95$\\
% thyroid-new& $23.25 \pm 1.36$ & $25.10 \pm 1.61$ & $\mathbf{22.50 \pm 3.08}$ & $28.10 \pm 4.03$ & $25.50 \pm 0.80$ & $24.95 \pm 0.72$\\
% movie& $20.90 \pm 1.96$ & $\mathbf{15.45 \pm 1.44}$ & $26.95 \pm 2.44$ & $25.60 \pm 2.49$ & $15.95 \pm 1.18$ & $22.35 \pm 2.06$\\
% theme& $29.95 \pm 1.83$ & $28.25 \pm 1.54$ & $33.65 \pm 1.04$ & $28.75 \pm 2.64$ & $28.60 \pm 1.28$ & $\mathbf{21.55 \pm 0.75}$\\
% entity& $24.15 \pm 1.87$ & $22.30 \pm 2.15$ & $30.85 \pm 1.48$ & $26.85 \pm 1.81$ & $\mathbf{21.60 \pm 1.26}$ & $24.10 \pm 2.05$\\
% % machine-cpu& $7.51e+04 \pm 7.29e+03$ & $\mathbf{3.65e+04 \pm 1.40e+04}$ & $1.73e+05 \pm 5.33e+04$ & $3.43e+05 \pm 9.65e+04$ & $4.21e+04 \pm 1.77e+04$ & $1.95e+05 \pm 5.29e+04$\\
% % fifa& $7.49e+03 \pm 2.60e+03$ & $6.42e+03 \pm 3.56e+03$ & $6.79e+03 \pm 2.13e+03$ & $1.66e+04 \pm 4.26e+03$ & $9.22e+03 \pm 4.67e+03$ & $\mathbf{2.06e+03 \pm 1.53e+03}$\\
% \end{tabular}
%     \caption{Falcon-7B}
%     \label{tab:Falcon-7B}
% \end{table}

==> addl_theory.tex <==
This section contains proofs of our main claims.


\subsection{Proof of \cref{lem:monotonicity}}
\label{sec:monotonicity proof-1}

Recall that the objective function is $f(S) = \bx_*\T \left(\bSigma_0^{-1} + \sigma^{-2} \sum_{i \in S} \bx_i \bx_i\T\right)^{-1} \bx_*$. Without loss of generality, let $\sigma^2 = 1$. Fix any $j \in [n] \setminus S$ and let $S_+ = S \cup \set{j}$. Then the objective value at $S_+$ can be written as
\begin{align*}
  f(S_+)
  = \bx_*\T \left(\bSigma_0^{-1} + \sum_{i \in S_+} \bx_i \bx_i\T\right)^{-1} \bx_*
  = \bx_*\T \left(\bA + \bx_j \bx_j\T\right)^{-1} \bx_*\,,
\end{align*}
where $\bA = \bSigma_0^{-1} + \sum_{i \in S} \bx_i \bx_i\T$. By the Sherman–Morrison formula, we have
\begin{align*}
  \left(\bA + \bx_j \bx_j\T\right)^{-1}
  = \bA^{-1} - \frac{\bA^{-1} \bx_j \bx_j\T \bA^{-1}}{1 + \bx_j\T \bA^{-1} \bx_j}\,.
\end{align*}
Now note that $\displaystyle \frac{\bA^{-1} \bx_j \bx_j\T \bA^{-1}}{1 + \bx_j\T \bA^{-1} \bx_j}$ is a positive semi-definite matrix for any $\bx_j$ and any positive semi-definite matrix $\bA$. As a result, $\displaystyle \bx_*\T \frac{\bA^{-1} \bx_j \bx_j\T \bA^{-1}}{1 + \bx_j\T \bA^{-1} \bx_j} \bx_* \geq 0$ holds for any $\bx_*$ and thus
\begin{align*}
  f(S_+)
  = \bx_*\T \bA^{-1} \bx_*\T -
  \bx_*\T \frac{\bA^{-1} \bx_j \bx_j\T \bA^{-1}}{1 + \bx_j\T \bA^{-1} \bx_j} \bx_*
  \leq \bx_*\T \bA^{-1} \bx_*\T
  = f(S)\,.
\end{align*}
This proves our claim.


\subsection{Proof of \cref{thm:go}}
\label{sec:go proof-1}

The proof is under the assumption that points can be partitioned as $\X = S \cup \bar{S}$. The set $S$ represents points that are close to $\bx_*$. It is convex and defined by $\alpha \geq 0$ such that $\bx\T \by \geq \alpha$ for all $\bx, \by \in S$. The set $\bar{S}$ represents points that are not close to $\bx_*$. It is defined $\beta \geq 0$ such that $\bx\T \by \leq \beta$ for all $\bx \in S$ and $\by \in \bar{S}$. The inverse of the covariance matrix after $t - 1$ observations is
\begin{align*}
  \widehat{\bSigma}_t^{-1}
  = \bLambda_t
  = \bI_d + \sum_{\ell = 1}^{t - 1} X_\ell X_\ell\T
  = \sum_{i = 1}^d \lambda_{t, i} \bv_{t, i} \bv_{t, i}\T\,.
\end{align*}
The latter is the eigendecomposition of $\bLambda_t$, where $\lambda_{t, i}$ is the $i$-th largest eigenvalue and $\bv_{t, i}$ is the corresponding eigenvector. Note that $\bLambda_t^{-1} = \sum_{i = 1}^d \lambda_{t, i}^{-1} \bv_{t, i} \bv_{t, i}\T$. To simplify exposition, we assume that all points have unit length. We analyze the eigenvalues of $\bLambda_t$ first.

\begin{lemma}
\label{lem:eigenvalues-1} For all $i \in [d]$, $1 \leq \lambda_{t, i} \leq t$. Moreover, let $X_\ell \in S$ hold for all $\ell \in [t - 1]$. Then $\lambda_{t, 1} \geq \alpha^2 (t - 1) + 1$.
\end{lemma}
\begin{proof}
The first claims follows directly from the definition of $\bLambda_t$ and that $\normw{X_\ell}{2} \leq 1$. The second claim is proved using the definition of the maximum eigenvalue,
\begin{align*}
  \lambda_{t, 1}
  = \bv_{t, 1}\T \bLambda_t \bv_{t, 1}
  \geq \bx_*\T \left(\bI_d + \sum_{\ell = 1}^{t - 1} X_\ell X_\ell\T\right) \bx_*
  \geq \alpha^2 (t - 1) + 1\,.
\end{align*}
The last inequality follows from $\bx_*\T X_\ell \geq \alpha$. This completes the proof.
\end{proof}

We continue with claims about the eigenvectors of $\bLambda_t$.

\begin{lemma}
\label{lem:eigenvectors-1} Let $X_\ell \in S$ hold for all $\ell \in [t - 1]$. Then $\bv_{t, 1} \in S$. Moreover, let $\beta \geq 1 - \alpha^2$. Then $\bv_{t, i} \in \bar{S}$ for all $i \geq 2$.
\end{lemma}
\begin{proof}
Since all $X_\ell \in S$ and $S$ is a convex set, $\bv_{t, 1} \in S$. Now take any $\bx \in S$ and $i \geq 2$, and note that
\begin{align*}
  (\bx\T \bv_{t, i})^2
  \leq \sum_{i = 2}^d (\bx\T \bv_{t, i})^2
  = 1 - (\bx\T \bv_{t, 1})^2
  \leq 1 - \alpha^2\,.
\end{align*}
We use that $\sum_{i = 1}^d (\bx\T \bv_{t, i})^2 = 1$ and $\bx\T \bv_{t, 1} \geq \alpha$. Therefore, when $\beta \geq 1 - \alpha^2$, we have $\bv_{t, i} \in \bar{S}$ for all $i \geq 2$.
\end{proof}

Our analysis has two parts. First, we bound the approximation error under the assumption that $X_\ell \in S$ holds for all $\ell \in [T]$. Second, we show how to choose $\alpha$ and $\beta$ to guarantee this. We start with the approximation error.

\begin{lemma}
\label{lem:approximation error-1} Let $X_\ell \in S$ hold for all $\ell \in [T]$. Then
\begin{align*}
  \bx_*\T \bLambda_{T + 1}^{-1} \bx_*
  \leq \frac{1}{\alpha^2 T + 1} + (1 - \alpha^2)\,.
\end{align*}
\end{lemma}
\begin{proof}
We start with
\begin{align*}
  \bx_*\T \bLambda_{T + 1}^{-1} \bx_*
  = \sum_{i = 1}^d \lambda_{T + 1, i}^{-1} \bx_*\T \bv_{T + 1, i} \bv_{T + 1, i}\T \bx_*
  \leq \frac{(\bx_*\T \bv_{T + 1, 1})^2}{\alpha^2 T + 1} +
  \sum_{i = 2}^d (\bx_*\T \bv_{T + 1, i})^2\,.
\end{align*}
The inequality uses lower bounds in \cref{lem:eigenvalues-1}. Then we apply $\bx_*\T \bv_{T + 1, 1} \leq 1$ and $\sum_{i = 2}^d (\bx_*\T \bv_{T + 1, i})^2 \leq 1 - \alpha^2$.
\end{proof}

Now we prove by induction that $X_\ell \in S$ holds for all $\ell \in [T]$.

\begin{lemma}
\label{lem:greedy point selection-1} Let $X_\ell \in S$ hold for all $\ell \in [t - 1]$. Suppose that $\displaystyle t \leq \frac{\alpha^2}{(\beta + \sqrt{2}) \beta d}$. Then $\bx_t \in S$.
\end{lemma}
\begin{proof}
Our algorithm chooses a point $\bx_t \in S$ when
\begin{align*}
  \frac{\bx_*\T \bLambda_t^{-1} \bx \bx\T \bLambda_t^{-1} \bx_*}
  {1 + \bx\T \bLambda_t^{-1} \bx}
  \geq \frac{\bx_*\T \bLambda_t^{-1} \by \by\T \bLambda_t^{-1} \bx_*}
  {1 + \by\T \bLambda_t^{-1} \by}
\end{align*}
holds for any $\bx \in S$ and $\by \in \bar{S}$. Since $0 \leq \bv\T \bLambda_t^{-1} \bv \leq 1$ for any $\normw{\bv}{2} \leq 1$, the above event occurs when
\begin{align*}
  (\bx_*\T \bLambda_t^{-1} \bx)^2
  = \bx_*\T \bLambda_t^{-1} \bx \bx\T \bLambda_t^{-1} \bx_*
  \geq 2 \bx_*\T \bLambda_t^{-1} \by \by\T \bLambda_t^{-1} \bx_*
  = 2 (\bx_*\T \bLambda_t^{-1} \by)^2\,.
\end{align*}
We start with an upper bound on the right-hand side,
\begin{align*}
  |\bx_*\T \bLambda_t^{-1} \by|
  \leq \sum_{i = 1}^d \lambda_{t, i}^{-1} |\bx_*\T \bv_{t, i} \bv_{t, i}\T \by|
  \leq \beta d\,.
\end{align*}
Here we use $\lambda_{t, i} \geq 1$ (\cref{lem:eigenvalues-1}), and that $\bv_{t, 1}\T \by \leq \beta$ and $\bx_*\T \bv_{t, i} \leq \beta$ when $i \geq 2$.

Now we bound the left-hand side as
\begin{align*}
  |\bx_*\T \bLambda_t^{-1} \bx|
  \geq \lambda_{t, 1}^{-1} |\bx_*\T \bv_{t, 1} \bv_{t, 1}\T \bx| -
  \sum_{i = 2}^d \lambda_{t, i}^{-1} |\bx_*\T \bv_{t, i} \bv_{t, i}\T \bx|
  \geq \frac{\alpha^2}{t} - \beta^2 d\,.
\end{align*}
To bound the first term, we use $\lambda_{t, 1} \leq t$, and that $\bx_*\T \bv_{t, 1} \geq \alpha$ and $\bv_{t, 1}\T \bx \geq \alpha$. To bound the second term, we use $\lambda_{t, i} \geq 1$, and that $\bx_*\T \bv_{t, i} \leq \beta$ and $\bv_{t, i}\T \bx \leq \beta$.

Now we chain all inequalities and get that our algorithm chooses a point $\bx_t \in S$ when
\begin{align*}
  t
  \leq \frac{\alpha^2}{(\beta + \sqrt{2}) \beta d}\,.
\end{align*}
This completes the proof.
\end{proof}

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided theoretical and empirical justification in the paper in the theory and experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our proposed algorithms \sal\ and \go\ are analyzed under specific assumptions on the label space and only for linear models, even though in practice they are applicable for non-linear models like \LLMs. We discuss this in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide all the assumptions and proofs in the main paper and Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides the full pseudocode of the proposed algorithms. All information about the experiments is provided in the experiment section. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is provided in the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of these details are provided in the main paper or in the additional experiment details in Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The standard deviation is reported in all the results in the experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide details of the \LLM\ models used in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the ethics guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the broader impact after the checklist.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is not applicable to this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite the \LLMs\ and the datasets used in the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is not applicable to this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is not applicable to this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is not applicable to this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

